Economics Arena for Large Language Models

Large language models (LLMs) have been extensively used as the backbones for general-purpose agents, and some economics literature suggest that LLMs are capable of playing various types of economics games. Following these works, to overcome the limitation of evaluating LLMs using static benchmarks, we propose to explore competitive games as an evaluation for LLMs to incorporate multi-players and dynamicise the environment. By varying the game history revealed to LLMs-based players, we find that most of LLMs are rational in that they play strategies that can increase their payoffs, but not as rational as indicated by Nash Equilibria (NEs). Moreover, when game history are available, certain types of LLMs, such as GPT-4, can converge faster to the NE strategies, which suggests higher rationality level in comparison to other models. In the meantime, certain types of LLMs can win more often when game history are available, and we argue that the winning rate reflects the reasoning ability with respect to the strategies of other players. Throughout all our experiments, we observe that the ability to strictly follow the game rules described by natural languages also vary among the LLMs we tested. In this work, we provide an economics arena for the LLMs research community as a dynamic simulation to test the above-mentioned abilities of LLMs, i.e. rationality, strategic reasoning ability, and instruction-following capability.

==> authorship.tex <==
\makeatletter
\newcommand{\myfnsymbol}[1]{%
  \expandafter\@myfnsymbol\csname c@#1\endcsname
}
% Mapping of how the \thanks symbols will be interpreted sequentially
\newcommand{\@myfnsymbol}[1]{%
  \ifcase #1
    % 0
  \or 1% 1
  \or 2% 2
  \or 3
  \or 4
  \or 5
  \or \TextOrMath{\textasteriskcentered}{*}% 6
  \or \TextOrMath{\textdagger}{\dagger}% 7
  \or \TextOrMath{\textdaggerdbl}{\ddagger}%8
  \fi
}
% Just to make things explicit in the code what it means
\newcommand{\uoe}{\@myfnsymbol{1}}
\newcommand{\bupt}{\@myfnsymbol{2}}
\newcommand{\hit}{\@myfnsymbol{3}}
\newcommand{\ubc}{\@myfnsymbol{4}}
\newcommand{\su}{\@myfnsymbol{5}}
\newcommand{\equalcontributor}{\@myfnsymbol{6}}
\newcommand{\correspondence}{\@myfnsymbol{7}}
\newcommand{\intern}{\@myfnsymbol{8}}
\def\thanks#1{\protected@xdef\@thanks{\@thanks
    \protect\footnotetext{#1}}
}

\makeatother


==> bak_results.tex <==
In this section, we illustrate our findings about the rationality and strategic reasoning ability of LLMs as defined in Section~\ref{sec:method}.
Herein, we ran experiments where players include \texttt{GPT-3.5-turbo}, \texttt{GPT-4}, \texttt{text-davinci-001}, \texttt{text-davinci-002}, \texttt{text-davinci-003}.
We have noted in the prompts whether rationality is explicitly required to separate the possibility of conflicting objectives, where strategies aiming at winning the game at all cost could differ from strategies that seek to maximise one's utility.
We have also varied the prompts used in the experiments to show that the metrics we proposed and the performance of LLMs under them are robust across the language of which the prompts were written in.

 \begin{figure}[t]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/second_price_auction_no_history.pdf}
        \caption{Second-Price Auction}
        \label{fig:results:rationality:multi_type:auction}
    \end{subfigure}
    ~
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=0.94\linewidth]{graphs/beauty_contest_no_history.pdf}
        \caption{Beauty Contest}
        \label{fig:results:rationality:multi_type:beauty}
    \end{subfigure}
    \caption{The average payoff of different agents (LLMs) in (a) second-price auction games and (b) beauty contest games.
    The results are averaged over 100 independent sessions of the games.
    Optimal payoff (indicated by the shadowed grey area) refers to the expected payoff when all agents make the bid strictly in conform with NE.
    }
    \label{fig:results:rationality:multi_type}
    \vspace{-1em}
\end{figure}

\subsection{(Non-maximal) Rational Behaviours of LLMs in Competitive Games}
\label{ssec:results:rationality}

Our first experiment is designed to compare the rationality degrees of various LLMs in our economics arena.
In this experimental set-up, LLMs are coined the role of agents, they compete in the economics arena simultaneously and are ranked by their payoffs.
To eliminate the possibility of reasoning about the strategies of other players in this experiment, we keep no game history in all of the games.
In the mean time, to ensure our results are statistically consistent, we run each game over 100 independent sessions\footnote{For the games ran with identical configurations, we refer the collection of them to be a single session.
For example, for 10 runs of the auction games where each agent has identical budget and private values, we call these 10 runs as a session.}, 
and collect the statistics about the average as well as the standard deviation of the payoffs obtained by the LLMs.
The results are given in the the Figure~\ref{fig:results:rationality:multi_type}.

As shown in Figure~\ref{fig:results:rationality:multi_type}, most of the LLMs we tested behave rationally in terms of attempting to maximise their utility, but not to the maximum degree of rationality as they did not achieve optimal payoffs.
For the second-price auction, most of the LLMs receive positive payoffs, but much less than optimal illustrated by the grey slashed area.
\texttt{text-davinci-001} does particularly bad and in fact incurs a huge loss comparable to the optimal.
Regarding the beauty contest game, since payoffs are non-negative in the set-up, we compare the actual payoffs obtained by different models with the expected payoffs under NEs, again illustrated by the grey slashed bars.
\texttt{text-davinci-001} almost never won in beauty contest games, whereas the averaged actual payoffs for \texttt{GPT-4} and \texttt{text-davinci-003} exceed the expected payoffs under NEs.
Intriguingly, in comparison with human subjects in the beauty contest game, who displayed bounded rationality and where most of them falls under step 1 and 2 of the reasoning iteration~\citep{nagel1995unraveling}, \texttt{GPT-4} and \texttt{text-davinci-003} show similar results.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/second_price_auction_no_history_self_compete.pdf}
        \caption{Second-Price Auction}
        \label{fig:results:rationality:single_type:auction}
    \end{subfigure}
    ~
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{graphs/beauty_contest_no_history_self_compete.pdf}
        \caption{Beauty Contest}
        \label{fig:results:rationality:single_type:beauty}
    \end{subfigure}
    \caption{The deviation from NE of agents (LLMs) in self-competing (a) second-price auction games and (b) beauty contest games.
    The results are sampled from 100 independent sessions for each type of agent, and empirical average is marked with darker colours.
    }
    \label{fig:results:rationality:single_type}
    \vspace{-1em}
\end{figure}

Overall, our results are in accordance with studies on economic rationality of LLMs in cooperative games~\citep{bauer2023decoding} and their behaviours in making budgetary decisions~\citep{chen2023emergence}, where 
However, it remains unclear if a LLM's irrationality could be due to itself or its opponents.
Take \texttt{GPT-4}'s performance in Figure~\ref{fig:results:rationality:multi_type:auction} for example, it might be surprising to see that its payoff is not the highest.
By checking out the logs of these games, we found that \texttt{GPT-4} failed to maximise its utility not because of itself but rather as a result of the overbidding strategies adopted by the other models, especially \texttt{text-davinci-001}.
As a consequence of other models behaving less rationally, \texttt{GPT-4} could be unable to make any positive payoff even if its private value associated with the item is the highest.
Therefore, to further investigate the source of the non-maximal payoff of each model, we let each LLM play with themselves, and check if this changes the rationality degree of their strategies.
The results are given in the following Figure~\ref{fig:results:rationality:single_type}.

From Figure~\ref{fig:results:rationality:single_type}, we can easily observe that particular LLMs behave more rationally when competing with themselves.
For instance, LLMs like \texttt{GPT-3.5-turbo}, \texttt{GPT-4}, \texttt{text-davinci-002} and \texttt{text-davinci-003} have obtained mean payoffs almost identical to the NE payoffs in self-competing auction games, indicating a high level of rationality of the respective models themselves, as well as that their previous non-maximal payoffs are more likely due to the strategies used by other models.
Meanwhile the distributions of \texttt{GPT-3.5-turbo} and \texttt{GPT-4} are more centralised than the other two, showing greater consistency of rationality performance.
In self-competing beauty context games, \texttt{GPT-4} also obtained an averaged payoff that is closest to the NE payoffs, which is an indication of higher rationality degree than others.

\subsection{Strategic Reasoning Ability of LLMs in Competitive Games}
\label{ssec:results:reasoning}

As illustrated in Section~\ref{ssec:method:reasoning}, in the following experiments, to test the strategic reasoning ability, we vary the available historical information in the experiments below.

\begin{figure}[b]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/second_price_auction_partial_history.pdf}
        \caption{Partial History}
        \label{fig:results:reasoning:auction:partial}
    \end{subfigure}
    ~
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=0.96\linewidth]{graphs/second_price_auction_full_history.pdf}
        \caption{Full History}
        \label{fig:results:reasoning:auction:full}
    \end{subfigure}
    ~
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=0.94\linewidth]{graphs/second_price_auction_full_history_self_compete.pdf}
        \caption{Full History, Self-Compete}
        \label{fig:results:reasoning:auction:single_type}
    \end{subfigure}
    \caption{The average payoff of agents (LLMs) in second-price auction games with 2 level of history given, i.e. partial history and full history.
    The results are averaged over 10 independent sessions of the games, and each session consists of 10 runs.
    Partial history merely contains the bidding prices of everyone in the last 5 runs, and full history contains private values of everyone on the basis of partial history. Self-Compete refers to the self-competing version of the game.
    }
    \label{fig:results:reasoning:auction}
\end{figure}

We first test how revealing the historical information changes the strategies of LLMs in our economics arena.
Note that the games we run are still single-round games, and the historical information are about the last several runs in the same sessions.
It is relatively straightforward to control the history information in beauty contest games. 
Since there are no private information, we simply vary the number of historical session logs to be incorporated into the prompts.
The auction games are a bit more complicated, as all agents have one public information, i.e. their bidding price, along with one private information, i.e the value they each associate with the auction item.
So, we set up the following two levels of available history information in auction games:
\begin{itemize}
    \item Partial history: only the bidding prices over a certain number of past sessions are available, where the number of sessions is controlled.
    \item Full history: both the bidding prices and the private values over a certain number of past sessions are available.
\end{itemize}
The results about agents' strategies when game history is available on auction games and beauty contest games are given in Figure~\ref{fig:results:reasoning:auction} and Figure~\ref{fig:results:reasoning:contest} respectively.

Comparing Figure~\ref{fig:results:rationality:multi_type:auction} with Figure~\ref{fig:results:reasoning:auction:partial} and Figure~\ref{fig:results:reasoning:auction:full}, we can see that available history actually lead to worse payoffs for most of the models, even \texttt{GPT-4}, especially in the partial history set-up.
We argue that this may be due to the complexity of prompts containing historical information in table form, which might make it harder to understand by the models, thus they cannot effectively utilise the information to bid, let alone correctly reason about other players' strategies given the prompts.
It is also possible that the variance of some LLMs's strategies is too large, thus inconsistent, which makes the inference about their strategies even more difficult.
So, to ensure that the models behave consistently over the sessions, we run the self-competing auction games, and make the full history available, where the results are given in Figure~\ref{fig:results:reasoning:auction:single_type}.
As can be seen, \texttt{GPT-4} obtains much better payoffs under this setup, which indicates that the failure of it in the above settings is more likely due to the inconsistency of other model's strategies.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/beauty_contest_full_history.pdf}
        \caption{Full History}
        \label{fig:results:reasoning:contest:full}
    \end{subfigure}
    ~
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=0.97\linewidth]{graphs/beauty_contest_full_history_self_compete.pdf}
        \caption{Full History, Self-Compete}
        \label{fig:results:reasoning:contest:uni_type}
    \end{subfigure}
    \caption{The process of one exemplary session over 10 runs in a beauty contest game with full history.
    Self-Compete refers to the self-competing version of the game.
    \vspace{-1em}
    }
    \label{fig:results:reasoning:contest}
    \vspace{-1em}
\end{figure}

More intriguingly, with more game information, \texttt{GPT-4} can almost perfectly fit the optimal strategy even if the other models behave irrationally, as can be seen by the overlap between the red and black dotted lines in Figure~\ref{fig:results:reasoning:contest:full}.
Considering that the strategies of other models are consistent and almost constant in beauty contest games, we argue that our results show that \texttt{GPT-4} can indeed reason about the strategies of other models.
So, to further investigate if this capability indeed arise from fitting the behaviours of other models, we set up the self-computing beauty contest game, where again multiple agents are playing against the agents backed by the same respective LLM, and the results are shown in Figure~\ref{fig:results:reasoning:contest:uni_type}.
It is straightforward to see that the models do change their strategies when the distribution over agent types change, especially \texttt{GPT-4} who converges very fast to the NE strategy in the game, i.e. guessing $0$.
Our results illustrate that models with stronger reasoning capability can indeed reason about other players' strategies, and win games more often by doing so.

\vspace{-0.5em}
\subsection{Natural Language Instruction Following Behaviours of LLMs}
\label{ssec:results:NLU}
\vspace{-0.5em}

During the above experiments, we also observed that certain LLMs cannot strictly follow the game instruction, i.e. either fail to give responses in the specified format or break the rules of the games, which reflects the ability of LLMs to follow instructions in natural languages.
So, we track the frequency of rule-breaking of each agent in each type of games, and the results are given in Table~\ref{tab:results:NLU:breaking_rule_results}.

\begin{table}[h]
\centering

\scalebox{0.85}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multirow{2}{*}[-0.5ex]
{\textbf{\begin{tabular}[c]{@{}c@{}}Game\\ Type\end{tabular}}} &
  \multirow{2}{*}[-0.5ex]{\textbf{\begin{tabular}[c]{@{}c@{}}History\\ Given\end{tabular}}} &
  \multicolumn{5}{c}{\textbf{Agent}} \\ \cmidrule(l){3-7} 
 &
   &
  \texttt{GPT-3.5}&
  \texttt{GPT-4}&
  \texttt{t-d-001} &
  \texttt{t-d-002} &
  \texttt{t-d-003} \\ \midrule\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Second-Price\\ Auction\end{tabular}} &
  No &
  \multicolumn{1}{c}{0\%(0/100)} &
  \multicolumn{1}{c}{0\%(0/100)} &
  \multicolumn{1}{c}{0\%(0/100)} &
  \multicolumn{1}{c}{6.00\%(6/100)} &
  0\%(0/100) \\ \cmidrule(l){2-7} 
 &
  Yes &
  \multicolumn{1}{c}{41.5\%(83/200)} &
  \multicolumn{1}{c}{17.0\%(34/200)} &
  \multicolumn{1}{c}{8.50\%(17/200)} &
  \multicolumn{1}{c}{10.5\%(21/200)} &
  1.00\%(2/200) \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Beauty\\ Contest\end{tabular}} &
  No &
  \multicolumn{1}{c}{0\%(0/100)} &
  \multicolumn{1}{c}{0\%(0/100)} &
  \multicolumn{1}{c}{0\%(0/100)} &
  \multicolumn{1}{c}{0\%(0/100)} &
  0\%(0/100) \\ \cmidrule(l){2-7} 
 &
  Yes &
  \multicolumn{1}{c}{0\%(0/200)} &
  \multicolumn{1}{c}{0\%(0/200)} &
  \multicolumn{1}{c}{0\%(0/200)} &
  \multicolumn{1}{c}{0\%(0/200)} &
  0.50\%(1/200) \\ \bottomrule
\end{tabular}
}

\caption{Frequency in the format of percentages of breaking rules by different LLMs during the experiments in our economics arena.
The results are obtained through tracking 100 runs without history and 200 runs with history of two kinds of game.
\texttt{t-d} is the abbreviation for ``text-davanci''.
\vspace{-1em}
}
\label{tab:results:NLU:breaking_rule_results}
\vspace{-0.5em}
\end{table}

By comparing the auction games and the beauty contests, we can see that the frequency of breaking rules in auctions is higher than the case of beauty contests.
By comparing the set-ups where history information is and is not available, we can also see the huge increase of breaking rules frequency.
Considering that prompts in auctions are more complex than the ones in beauty contests as well as the fact that adding history information makes the prompts even more complicated, we argue that the certain types of LLMs fail to follow the instructions because they cannot understand the prompts with higher complexity.
Therefore, we argue that our economics arena can also reflect the ability of LLMs to strictly follow the natural language instructions.

\vspace{-0.5em}

==> discussion.tex <==
\vspace{-1em}

% While we explored the two types of competitive games and show interesting results, we also recognise that the number of games included in this paper is limited, and the variations in the set-ups are restricted.
% There are potential to generalise and refine our metrics further by investigating more forms of games.

%  Another possible limitation lays in the sensitivity of results to key elements in prompts.
%  For instance, LLMs' behaviours could be strongly reliant on the explicit requirement of rationality in the prompts, without which, LLMs might have other objectives, such as winning the games at all cost, that could lead to conflicting results or higher frequency of rule breaking.
%  Furthermore, it is also possible that our observations are restricted to the language environment that was picked.
%  Following studies on Wittgenstein's formalisation of language as a set of rules or practices~\citep{malcolm1989wittgenstein}, human following different rules could behave differently as according to their language settings.
%  Since LLMs are trained on large amount of human-generated data, by varying the language prompts, we could effectively separate and compare the metrics measure by different groups of ``rule-followers".
%  The degree of rationality and strategic reasoning ability could differ for the same LLM across the language settings, which could provide another dimension to evaluate the LLMs.
%  While this has not been analysed in this paper, it is an interesting direction and is intended to be explored.

%  Last but not the least, a question that is still open to discussion is how we can combine the game idea with the real world applications.
%  In practical scenarios, we often do not have the ground-truth, (i.e. the knowledge of NE strategies), therefore it would be difficult to analyse how rational LLMs are in those situations.
%  However, the economics games provide a simplified environment to evaluate the models, and could be compared with the experimental results of human subjects to check if they could perform better, more rationally and more strategically.
%  This might highlight a case for real life application, where following advice of certain more advanced LLMs could lead to better outcome.
%  Nonetheless, these games serve as the basis before evaluating more complicated models that have theoretical predictions and closer to real world scenarios.

% \vspace{-0.5em}

%1) limited economics games, and set-ups. we may want to generalise our idea thus it can be applied to more forms of games, not necessarily certain time of economics games.
%2) sensitivity of the results to key elements in prompts, e.g. whether rationality is explicitly required, CoT, language
%3) to real life scenarios, we do not always have ground-truth (NEs), so how can we combine the game idea with the real life applications is still unclear

==> instruction.tex <==
\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.
